Simple and Efficient Confidence Score for Grading Whole Slide Images

Grading precancerous lesions on whole slide images is a challenging task: the continuous space of morphological phenotypes makes clear-cut decisions between different grades often difficult, leading to low inter- and intra-rater agreements. More and more Artificial Intelligence (AI) algorithms are developed to help pathologists perform and standardize their diagnosis. However, those models can render their prediction without consideration of the ambiguity of the classes and can fail without notice which prevent their wider acceptance in a clinical context. In this paper, we propose a new score to measure the confidence of AI models in grading tasks. Our confidence score is specifically adapted to ordinal output variables, is versatile and does not require extra training or additional inferences nor particular architecture changes. Comparison to other popular techniques such as Monte Carlo Dropout and deep ensembles shows that our method provides state-of-the art results, while being simpler, more versatile and less computationally intensive. The score is also easily interpretable and consistent with real life hesitations of pathologists. We show that the score is capable of accurately identifying mispredicted slides and that accuracy for high confidence decisions is significantly higher than for low-confidence decisions (gap in AUC of 17.1% on the test set). We believe that the proposed confidence score could be leveraged by pathologists directly in their workflow and assist them on difficult tasks such as grading precancerous lesions.

==> hacks/many-authors-hack.tex <==
% This hack should not be needed anynore as the issue has been fixed upstream in JMLR v1.26 (2020-01-31)
% https://github.com/MIDL-Conference/MIDLLatexTemplate/issues/8
% https://www.dickimaw-books.com/bugtracker.php?action=view&key=141

%\begin{comment}
\makeatletter
% hack the footer of the title page as it doesn't seem to automatically use the et al. version when spanning acros multiple pages
\renewcommand*{\@titlefoot}{\scriptsize\copyright\space\@jmlryear
    \ifanonsubmission
    \space Author(s) names withheld.\hfill
    \else
    \space \@firstauthor\space \emph{et al}.\hfill
    \@reprint
    \fi
  }
\makeatother
%\end{comment}

% \begin{comment}
\makeatletter
% remove the vbox in @jmlrmaketitle which prevents the text to be split across several pages
\renewcommand{\@jmlrmaketitle}{
  % specify the page style in case it spans over several pages. Not sure why this is needed
  \thispagestyle{jmlrtps}%
  % define a new label for the first page as otherwise it starts from 2 in the header
  \label{jmlrstartnew}%
  % hack the spacing to mimick what happens with a vbox
  \null\vspace{-\parindent}\vspace{-2pt}{
  \hsize\textwidth
  \linewidth\hsize
 \jmlrpretitle
  {%
    \def\titletag##1{##1}%
    \@title
  }%
 \jmlrposttitle
 \jmlrpreauthor \@author \jmlrpostauthor
}
% hack the spacing to mimick what happens with a vbox
\vspace{2pt}
}
\makeatother
%\end{comment}

%\begin{comment}
\makeatletter
% hack the footer to use the new counter
\renewcommand*\@jmlrpages{\pageref{jmlrstartnew}--\pageref{jmlrend}}
\makeatother
%\end{comment}

==> sections/table_full.tex <==

\begin{landscape}
\begin{table*}[htbp]
% % The first argument is the label.
% % The caption goes in the second argument, and the table contents
% % go in the third argument.
\floatconts
{tab:table2}%
{\caption{Stratification of the gold standard test set between high confidence and low confidence slides. Ensembling predictions from the 5 folds cross validation trainings and bootstraped.}}%
{
\begin{adjustbox}{width=1.5\textwidth}
\begin{tabular}{cccccccccccccccc}
\textbf{threshold= median}      & \multicolumn{3}{c}{\textbf{AUC (Average on 4 classes)}}                                      & \multicolumn{3}{c}{\textbf{NPV Carcinoma (3)}}                                               & \multicolumn{3}{c}{\textbf{NPV Abnormal (1+2+3)}}                                                                              & \multicolumn{3}{c}{\textbf{AUC Carcinoma  (3)}}                                              & \multicolumn{3}{c}{\textbf{AUC Abnormal (1+2+3)}}                                            \\
\textit{1000 bootstraps}        & \textit{\textbf{Low Confidence}} & \textit{\textbf{High Confidence}} & \textit{\textbf{Gap}} & \textit{\textbf{Low Confidence}} & \textit{\textbf{High Confidence}} & \textit{\textbf{Gap}} & \textit{\textbf{Low Confidence}}                                   & \textit{\textbf{High Confidence}} & \textit{\textbf{Gap}} & \textit{\textbf{Low Confidence}} & \textit{\textbf{High Confidence}} & \textit{\textbf{Gap}} & \textit{\textbf{Low Confidence}} & \textit{\textbf{High Confidence}} & \textit{\textbf{Gap}} \\
\textbf{MC-Dropout}             & 0.842 {[}0.78, 0.9{]}            & 0.884 {[}0.823, 0.938{]}          & 4,2\%                 & 0.95 {[}0.87, 1.0{]}             & 0.936 {[}0.86, 1.0{]}             & -1,4\%                & 0.664 {[}0.364, 0.917{]}                                           & 0.733 {[}0.47, 1.0{]}             & 6,90\%                & 0.953 {[}0.893, 0.997{]}         & 0.936 {[}0.857, 1.0{]}            & -1,70\%               & 0.825 {[}0.708, 0.919{]}         & 0.948 {[}0.889, 0.99{]}           & 12,30\%               \\
\textbf{Raw risk (SOSR)}        & 0,797 {[}0.719, 0.862{]}         & 0,934 {[}0.882, 0.978{]}          & 13,70\%               & 0,92 {[}0.847, 0.984{]}          & \textbf{1 {[}1.0, 1.0{]}}         & \textbf{8,00\%}       & 0,621 {[}0.25, 1.0{]}                                              & 0,742 {[}0.524, 0.938{]}          & 12,10\%               & 0,891 {[}0.768, 0.988{]}         & 0,979 {[}0.939, 1.0{]}            & \textbf{8,80\%}       & 0,737 {[}0.577, 0.875{]}         & 0,968 {[}0.922, 1.0{]}            & 23,10\%               \\
\textbf{Deep Ensembling}        & 0.79 {[}0.719, 0.858{]}          & 0.928 {[}0.879, 0.978{]}          & 13,8\%                & 0.938  {[}0.879, 0.985{]}        & \textbf{1.0 {[}1.0, 1.0{]}}       & 6,2\%                 & 0.54 {[}0.222, 0.819{]}                                            & 0.809 {[}0.588, 1.0{]}            & 26,90\%               & 0.911 {[}0.8, 0.991{]}           & \textbf{0.982 {[}0.942, 1.0{]}}   & 7,10\%                & 0.722 {[}0.567, 0.849{]}         & 0.968 {[}0.916, 1.0{]}            & 24,60\%               \\
\textbf{Grade Sensitive (Ours)} & 0.77 {[}0.689, 0.84{]}           & \textbf{0.941 {[}0.902, 0.977{]}} & \textbf{17,1\%}       & 0.92 {[}0.848, 0.983{]}          & \textbf{1.0 {[}1.0, 1.0{]}}       & \textbf{8,0\%}        & \begin{tabular}[c]{@{}c@{}}0.496\\ {[}0.214, 0.778{]}\end{tabular} & \textbf{0.867 {[}0.667, 1.0{]}}   & \textbf{37,10\%}      & 0.915 {[}0.815, 0.989{]}         & 0.98 {[}0.942, 1.0{]}             & 6,50\%                & 0.718  {[}0.562, 0.852{]}        & \textbf{0.974 {[}0.931, 1.0{]}}   & \textbf{25,60\%}     
\end{tabular}
\end{adjustbox}
}
\end{table*}
\end{landscape}
